Folksonomication: Predicting Tags for Movies from Plot Synopses Using Emotion Flow Encoded Neural Network

Folksonomy of movies covers a wide range of heterogeneous information about movies, like the genre, plot structure, visual experiences, soundtracks, metadata, and emotional experiences from watching a movie. Being able to automatically generate or predict tags for movies can help recommendation engines improve retrieval of similar movies, and help viewers know what to expect from a movie in advance. In this work, we explore the problem of creating tags for movies from plot synopses. We propose a novel neural network model that merges information from synopses and emotion flows throughout the plots to predict a set of tags for movies. We compare our system with multiple baselines and found that the addition of emotion flows boosts the performance of the network by learning ~18\% more tags than a traditional machine learning system.

==> sections_data/results_section.tex <==
% Table \ref{tab:tab_results_test} shows the performances of the experimented models on validation data by selecting top 3 and 5 tags. We will mainly discuss the results achieved by selecting top 5 tags for better clarity in the rest of the paper.\\

% \input{tables/results_table1.tex}
% \input{tables/test_results.tex}

% \noindent{\textbf{Hand-crafted features:}} Lexical features seem to be stronger among all the hand-crafted features. All of them beat the baselines. The best micro F1 0.378 is achieved by the character n-grams. Several individual features and feature combinations achieved micro F1 around 0.37. So the next metric to look at is the tags learned (TL) metric that helps to know how many tags are being learned by the models. Results show that, the model that learned the highest number of tags uses all the hand-crafted features combinations. It achieved micro F1 score of 0.369 and learned around 40 tags. Similar performance is also achieved by only using the lexical features. Word and character n-grams combined with the skip-grams helped to learn around 38 tags with similar micro F1.\\
% We observe interesting results using sentiment features by dividing them into chunks. Dividing the synopses into chunks based on the length of the texts in words and using sentiment features for each chunk helps the model to utilize sentiment information in different portions of the story more effectively. As the bag of concepts (BoC) features are almost a subset of the word n-grams features, they show better performance than the concept scores. Combination of them results a small improvement in the tags learned metrics. We can see from the results that, using 3 chunks achieve the optimal results as the micro F1 starts to drop if we go beyond 3 chunks where learned tags remains almost similar.\\
% Although micro F1 achieved by word embedding is good compared to the lexical features, tags learned by using it is lower and it is similar to the tags learned using semantic frames.

% Observing the micro F1 scores for all of the reported systems suggest that, predicting tags from the written plot synopses is a very difficult problem. Challenge lies in improving the micro F1 by making correct prediction simultaneously increasing the learned tags my the system.

% \noindent{\textbf{Chunk based Sentiment Representation: }}Different parts of narratives portray different types of experiences. We hypothesize that dividing the narratives into chunks and capturing sentiments features can help better represent the flow of sentiments in different parts of the stories. So we experiment by dividing the texts into 3, 4 and 5 chunks based on number of sentences and extracting the sentiment and emotion features for each chunks. Results show that, when sentiment and emotion features are represented by chunking the plots into several parts, the model can learn more tags with a small improvement in tag recall. 

% \noindent{\textbf{Performance of Neural Network Models: }}






==> tables/data_statistics.tex <==
\begin{table}[t]
\centering
\scalebox{0.9}{
\begin{tabular}{|l|r|}
\hline
Total Plot Synopses                      & 14,828 \\
Total Tags                               & 71     \\ \hline
Average tags per movie                   & 2.98   \\ 
Median value of tags per movie       	 	 & 2     \\ 
STD of tags for a movie       	 	 & 2.60     \\ 
Lowest number of tags for a movie         & 1      \\ 
Highest number of tags for a movie       & 26     \\ \hline
Average sentences per synopsis    		 & 43.59  \\ 
Median value of sentences per synopsis    	 & 32  \\ 
STD of sentences per synopsis    	 	 & 47.5  \\ 
Highest number of sentences in a synopsis & 1,434   \\ 
Lowest number of sentences in a synopsis  & 10     \\ \hline
Average words per synopsis        & 986.47 \\ 
Median value of words per synopsis        & 728 \\ 
STD of words per synopsis        & 966.16 \\ 
Highest number of words in a synopsis     & 13,576  \\ 
Lowest number of words in a synopsis      & 72     \\ \hline 
\end{tabular}
}
\caption{\small Brief Statistics of the Dataset.}
\label{tab_data_stat_table}
\end{table}

==> tables/front_page_examples.tex <==
\begin{table}[!hbtp]
\centering
% \small
% \begin{tabular}{|p{0.2\textwidth}|p{0.23\textwidth}|p{0.23\textwidth}|p{0.23\textwidth}|}
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline
\textbf{IMDB ID} & \makecell{\textbf{Movie Title}} & \makecell{\textbf{Predicted Tags}}\\ \hline

tt0133093 &
\makecell{\textbf{The Matrix}} &
\makecell{\textcolor{blue}{murder}, \textcolor{blue}{mystery}, \textcolor{blue}{sci-fi},\\ \textcolor{red}{suspenseful}, \textcolor{blue}{violence}} \\ 
\hline

tt0233298 &
\makecell{\textbf{Batman Beyond:}\\\textbf{Return of the Joker}} &
\makecell{\textcolor{blue}{comedy}, \textcolor{blue}{cult}, \textcolor{red}{dark},\\\textcolor{blue}{murder}, \textcolor{blue}{violence}} \\
\hline

tt0309820 &
\makecell{\textbf{Luther}} &
\makecell{\textcolor{red}{christian film}, \textcolor{red}{historical},\\\textcolor{red}{intrigue}, \textcolor{blue}{murder}, \textcolor{blue}{violence}} \\
\hline


\end{tabular}
% }
\caption{\small Example of predicted tags from the plot synopses of three movies. Blue and red labels indicate true positives and false positives respectively.}\label{tab:tab_tags_script_plot_example}
\end{table}
